Approximating the Core via Iterative Coalition Sampling

The core is a central solution concept in cooperative game theory, defined as the set of feasible allocations or payments such that no subset of agents has incentive to break away and form their own subgroup or coalition. However, it has long been known that the core (and approximations, such as the least-core) are hard to compute. This limits our ability to analyze cooperative games in general, and to fully embrace cooperative game theory contributions in domains such as explainable AI (XAI), where the core can complement the Shapley values to identify influential features or instances supporting predictions by black-box models. We propose novel iterative algorithms for computing variants of the core, which avoid the computational bottleneck of many other approaches; namely solving large linear programs. As such, they scale better to very large problems as we demonstrate across different classes of cooperative games, including weighted voting games, induced subgraph games, and marginal contribution networks. We also explore our algorithms in the context of XAI, providing further evidence of the power of the core for such applications.

==> convergenceproofs.tex <==


\section{Convergence Proofs}
\label{sect:theoretical_analysis_convergence}

Given that we have bound all the decision variables in each algorithm, the gradients and monotone operators (i.e., $\frac{d_c}{\vert C \vert} c$ and $F(x)$) are likewise bounded by inspection. In addition, the number of possible constraints is finite, therefore, the expected variances and norms of the gradients and monotone operators are finite for any batch size $B$.


\begin{theorem}
Let $v : 2^I \rightarrow \mathbb{R}$ be a characteristic function. Given an $\epsilon$ and assuming the $\epsilon$-core exists, Algorithm~\ref{alg:iterative_proj} converges to an $\epsilon$-core imputation asymptotically, i.e.: $\lim_{T \rightarrow \infty} p_T \rightarrow \epsilon$-core$(v)$.
\end{theorem}
\begin{proof}
We can appeal directly to classical convergence results of the von Neumann-Halperin cyclic projections algorithm~\citep{badea2016ritt}.
\end{proof}

\begin{theorem}
Let $v : 2^I \rightarrow \mathbb{R}$ be a characteristic function. Given an $\epsilon$ and assuming the $\epsilon$-core exists, Algorithm~\ref{alg:stochastic_gradient} converges to an $\epsilon$-core imputation in expectation at a rate of $\mathcal{O}(T^{-1/4})$.
\end{theorem}
\begin{proof}
We can appeal directly to convergence rates of stochastic projected subgradient algorithms for convex optimization~\cite{davis2018stochastic} given we have already argued above that the expectation of the squared gradient norm is bounded. These rates prove Algorithm~\ref{alg:stochastic_gradient} converges to a stationary point with $\mathcal{O}(1/\sqrt{T})$ expected squared gradient norm. Recall~\eqref{eqn:subgrad} to determine that the squared gradient is proportional to $d_c^2$. Therefore, the violation of the core constraints decays as $\mathcal{O}(T^{-1/4})$.
\end{proof}




\begin{theorem}
Let $v : 2^I \rightarrow \mathbb{R}$ be a characteristic function. Algorithm~\ref{alg:lagrangian_core} reduces the duality gap $\max_{\mu'} \mathcal{L}(p, \epsilon, \mu') - \min_{p', \epsilon'} \mathcal{L}(p', \epsilon', \mu)$ at a rate of $\mathcal{O}(1/\sqrt{T})$.
\end{theorem}
\begin{proof}
We can appeal directly to convergence rates of mirror prox algorithms for monotone variational inequalities~\citep{juditsky2011solving} given we have already argued above that the norm of the monotone map and its variance are both finite.
\end{proof}


